An ensemble approach to the study of the emergence of metabolic and proliferative disorders via Flux Balance Analysis

An extensive rewiring of cell metabolism supports enhanced proliferation in cancer cells. We propose a systems level approach to describe this phenomenon based on Flux Balance Analysis (FBA). The approach does not explicit a cell biomass formation reaction to be maximized, but takes into account an ensemble of alternative flux distributions that match the cancer metabolic rewiring (CMR) phenotype description. The underlying concept is that the analysis the common/distinguishing properties of the ensemble can provide indications on how CMR is achieved and sustained and thus on how it can be controlled.

==> eptcsdata.tex <==
\providecommand{\firstpage}{92}
\providecommand{\publicationstatus}{A. Graudenzi, G. Caravagna, G. Mauri, M. Antoniotti (Eds.): \\Wivace 2013 - Italian Workshop on \\Artificial Life and Evolutionary Computation\\
EPTCS 130, 2013, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.130.15}{10.4204/EPTCS.130.15}}
\pdfoutput=1

